Kinematic analysis of an Ultra-Strong MgII absorber at z~1.13 linking to Circumgalactic Gas Structures

We present a spectroscopic and imaging analysis of the $z_{gal} \approx 1.1334$ ultra-strong MgII absorption system identified in the $VLT$/UVES spectrum of a background quasar located at $\rho \approx 18$ kpc from a star-forming galaxy. Low ionization metal lines like MgI, FeII, and CaII are also detected for this absorber. The HI lines are outside of the wavelength coverage. The MgII has a rest-frame equivalent width of $W_r(2796) =3.185 +/- 0.032 A^{\circ} $, with the absorption spread across $\Delta v \approx 460$ km~s$^{-1}$ in several components. A component-by-component ionization modeling shows several of these components having solar and higher metallicities. The models also predict a total HI column density of $log[N(HI)/cm^{-2}] \approx 22.5$, consistent with ultra-strong MgII absorbers being sub-Damped Lyman Alpha and Damped Lyman Alpha systems. The absorber is well within the virial radius of the nearest galaxy which has a stellar mass $M_* = 4.7 \times 10^{10}$~M$_\odot$, and a star formation rate of $\approx 8.3$~M$_\odot$~yr$^{-1}$. The absorption is along the projected major axis of the galaxy with a velocity spread that is wider than the galaxy's disk rotation. From the kinematic analysis of the absorber and the galaxy, the origin of the absorption can be attributed to a combination of circumgalactic gas structures, some corotating with the disk and the rest at line-of-sight velocities outside of the disk rotation.

==> tables/Properties.tex <==
$-230.01_{-0.07}^{+0.15}$ & $-1.01_{-0.99}^{+0.75}$ & $-1.90_{-0.28}^{+0.25}$ & $16.46_{-0.69}^{+0.86}$ & $4.20_{-0.08}^{+0.07}$ & $-0.75_{-0.76}^{+0.79}$ & $3.1_{-0.9}^{+0.8}$ & $16.3_{-1.4}^{+1.3}$ & $16.6_{-1.3}^{+1.2}$\\[2pt]
$-214.09_{-0.07}^{+0.10}$ & $0.59_{-0.17}^{+0.10}$ & $-1.88_{-0.02}^{+0.02}$ & $15.90_{-0.11}^{+0.17}$ & $3.45_{-0.20}^{+0.27}$ & $-1.91_{-0.29}^{+0.35}$ & $5.9_{-0.2}^{+0.2}$ & $6.8_{-1.4}^{+2.5}$ & $9.0_{-1.0}^{+1.9}$\\[2pt]
$-199.00_{-0.12}^{+0.13}$ & $0.51_{-0.09}^{+0.09}$ & $-1.82_{-0.01}^{+0.01}$ & $16.00_{-0.10}^{+0.10}$ & $3.54_{-0.14}^{+0.16}$ & $-1.87_{-0.19}^{+0.21}$ & $6.7_{-0.2}^{+0.2}$ & $7.6_{-1.1}^{+1.5}$ & $10.1_{-0.8}^{+1.1}$\\[2pt]
$-181.61_{-0.15}^{+0.07}$ & $0.48_{-0.15}^{+0.14}$ & $-1.68_{-0.04}^{+0.07}$ & $15.44_{-0.14}^{+0.16}$ & $3.53_{-0.21}^{+0.19}$ & $-2.65_{-0.36}^{+0.28}$ & $9.0_{-0.3}^{+0.3}$ & $7.5_{-1.6}^{+1.9}$ & $11.7_{-0.9}^{+1.2}$\\[2pt]
$-157.45_{-0.10}^{+0.09}$ & $-1.37_{-0.39}^{+0.48}$ & $0.43_{-0.56}^{+0.62}$ & $17.83_{-0.68}^{+0.53}$ & $3.96_{-0.03}^{+0.04}$ & $-3.88_{-0.52}^{+0.58}$ & $0.6_{-0.4}^{+0.5}$ & $12.3_{-0.5}^{+0.5}$ & $12.3_{-0.5}^{+0.5}$\\[2pt]
$-128.07_{-0.00}^{+0.00}$ & $0.56_{-0.01}^{+0.01}$ & $-1.96_{-0.01}^{+0.01}$ & $15.26_{-0.05}^{+0.05}$ & $3.52_{-0.02}^{+0.02}$ & $-2.36_{-0.07}^{+0.06}$ & $11.0_{-0.0}^{+0.0}$ & $7.4_{-0.2}^{+0.2}$ & $13.3_{-0.1}^{+0.1}$\\[2pt]
$-111.87_{-0.00}^{+0.00}$ & $0.43_{-0.02}^{+0.03}$ & $-1.80_{-0.00}^{+0.00}$ & $16.13_{-0.06}^{+0.05}$ & $3.67_{-0.05}^{+0.03}$ & $-1.70_{-0.07}^{+0.07}$ & $8.8_{-0.0}^{+0.0}$ & $8.8_{-0.5}^{+0.4}$ & $12.4_{-0.3}^{+0.3}$\\[2pt]
$-94.97_{-0.00}^{+0.00}$ & $1.50_{-0.02}^{+0.03}$ & $-3.01_{-0.01}^{+0.02}$ & $14.99_{-0.06}^{+0.06}$ & $2.72_{-0.02}^{+0.02}$ & $-1.10_{-0.10}^{+0.07}$ & $6.4_{-0.0}^{+0.0}$ & $2.9_{-0.1}^{+0.1}$ & $7.0_{-0.0}^{+0.0}$\\[2pt]
$-81.59_{-0.02}^{+0.01}$ & $1.40_{-0.01}^{+0.01}$ & $-2.74_{-0.02}^{+0.02}$ & $15.01_{-0.05}^{+0.05}$ & $2.62_{-0.02}^{+0.01}$ & $-1.68_{-0.08}^{+0.08}$ & $8.8_{-0.0}^{+0.0}$ & $2.6_{-0.1}^{+0.0}$ & $9.2_{-0.1}^{+0.1}$\\[2pt]
$-68.39_{-0.02}^{+0.02}$ & $1.02_{-0.03}^{+0.03}$ & $-2.44_{-0.04}^{+0.03}$ & $14.62_{-0.06}^{+0.06}$ & $2.85_{-0.03}^{+0.02}$ & $-2.48_{-0.06}^{+0.06}$ & $1.0_{-0.1}^{+0.1}$ & $3.4_{-0.1}^{+0.1}$ & $3.6_{-0.1}^{+0.1}$\\[2pt]
$-46.83_{-0.01}^{+0.01}$ & $0.45_{-0.01}^{+0.02}$ & $-1.80_{-0.00}^{+0.00}$ & $16.35_{-0.05}^{+0.05}$ & $3.64_{-0.03}^{+0.01}$ & $-1.51_{-0.06}^{+0.05}$ & $14.4_{-0.0}^{+0.0}$ & $8.4_{-0.3}^{+0.1}$ & $16.7_{-0.1}^{+0.1}$\\[2pt]
$-27.16_{-0.04}^{+0.04}$ & $0.48_{-0.01}^{+0.01}$ & $-1.08_{-0.01}^{+0.01}$ & $17.33_{-0.05}^{+0.05}$ & $3.41_{-0.01}^{+0.01}$ & $-2.09_{-0.05}^{+0.05}$ & $4.9_{-0.0}^{+0.0}$ & $6.5_{-0.1}^{+0.1}$ & $8.2_{-0.1}^{+0.0}$\\[2pt]
$-15.46_{-0.03}^{+0.07}$ & $-1.71_{-0.02}^{+0.02}$ & $-2.38_{-0.03}^{+0.06}$ & $20.04_{-0.05}^{+0.05}$ & $4.30_{-0.03}^{+0.02}$ & $1.71_{-0.13}^{+0.09}$ & $7.6_{-0.0}^{+0.1}$ & $18.1_{-0.5}^{+0.4}$ & $19.7_{-0.5}^{+0.4}$\\[2pt]
$-1.77_{-0.01}^{+0.01}$ & $-3.73_{-0.03}^{+0.02}$ & $-1.47_{-0.02}^{+0.01}$ & $21.84_{-0.05}^{+0.06}$ & $3.99_{-0.00}^{+0.00}$ & $1.86_{-0.06}^{+0.06}$ & $4.7_{-0.1}^{+0.0}$ & $12.7_{-0.0}^{+0.0}$ & $13.6_{-0.0}^{+0.0}$\\[2pt]
$17.78_{-0.06}^{+0.08}$ & $-3.50_{-0.20}^{+0.14}$ & $0.40_{-0.02}^{+0.02}$ & $21.36_{-0.15}^{+0.20}$ & $2.92_{-0.06}^{+0.04}$ & $-0.53_{-0.15}^{+0.21}$ & $10.9_{-0.1}^{+0.1}$ & $3.7_{-0.2}^{+0.2}$ & $11.5_{-0.2}^{+0.1}$\\[2pt]
$41.42_{-0.01}^{+0.01}$ & $0.58_{-0.01}^{+0.01}$ & $-1.97_{-0.01}^{+0.01}$ & $16.35_{-0.05}^{+0.05}$ & $3.45_{-0.02}^{+0.02}$ & $-1.29_{-0.06}^{+0.06}$ & $4.1_{-0.0}^{+0.0}$ & $6.8_{-0.2}^{+0.1}$ & $7.9_{-0.1}^{+0.1}$\\[2pt]
$58.58_{-0.10}^{+0.06}$ & $-3.62_{-0.02}^{+0.05}$ & $-1.68_{-0.05}^{+0.04}$ & $21.72_{-0.07}^{+0.06}$ & $4.01_{-0.00}^{+0.00}$ & $1.96_{-0.06}^{+0.06}$ & $7.0_{-0.1}^{+0.1}$ & $13.0_{-0.0}^{+0.0}$ & $14.7_{-0.0}^{+0.0}$\\[2pt]
$74.09_{-0.12}^{+0.08}$ & $-3.06_{-0.02}^{+0.03}$ & $-2.12_{-0.02}^{+0.01}$ & $21.08_{-0.06}^{+0.05}$ & $4.08_{-0.00}^{+0.01}$ & $1.87_{-0.06}^{+0.06}$ & $5.8_{-0.2}^{+0.3}$ & $14.1_{-0.0}^{+0.1}$ & $15.2_{-0.1}^{+0.2}$\\[2pt]
$82.34_{-0.03}^{+0.02}$ & $0.19_{-0.01}^{+0.02}$ & $-1.40_{-0.07}^{+0.05}$ & $16.83_{-0.05}^{+0.05}$ & $3.78_{-0.01}^{+0.01}$ & $-1.69_{-0.12}^{+0.14}$ & $2.8_{-0.1}^{+0.1}$ & $10.0_{-0.1}^{+0.1}$ & $10.4_{-0.1}^{+0.1}$\\[2pt]
$91.24_{-0.06}^{+0.14}$ & $-3.99_{-0.00}^{+0.01}$ & $-1.68_{-0.02}^{+0.02}$ & $21.73_{-0.05}^{+0.05}$ & $4.01_{-0.00}^{+0.00}$ & $1.97_{-0.05}^{+0.05}$ & $5.1_{-0.1}^{+0.1}$ & $13.0_{-0.0}^{+0.0}$ & $13.9_{-0.0}^{+0.0}$\\[2pt]
$104.90_{-0.07}^{+0.11}$ & $-3.96_{-0.02}^{+0.01}$ & $0.09_{-0.03}^{+0.02}$ & $21.77_{-0.05}^{+0.05}$ & $3.21_{-0.03}^{+0.04}$ & $0.20_{-0.06}^{+0.06}$ & $9.6_{-0.1}^{+0.1}$ & $5.2_{-0.2}^{+0.2}$ & $10.9_{-0.1}^{+0.1}$\\[2pt]
$126.21_{-0.01}^{+0.02}$ & $0.55_{-0.02}^{+0.02}$ & $-1.89_{-0.01}^{+0.01}$ & $15.97_{-0.05}^{+0.05}$ & $3.51_{-0.03}^{+0.03}$ & $-1.80_{-0.06}^{+0.06}$ & $6.2_{-0.0}^{+0.0}$ & $7.3_{-0.2}^{+0.2}$ & $9.5_{-0.2}^{+0.2}$\\[2pt]
$147.98_{-0.03}^{+0.05}$ & $-3.99_{-0.01}^{+0.02}$ & $-1.50_{-0.04}^{+0.03}$ & $21.71_{-0.05}^{+0.05}$ & $4.00_{-0.00}^{+0.00}$ & $1.77_{-0.07}^{+0.07}$ & $6.1_{-0.0}^{+0.0}$ & $12.8_{-0.0}^{+0.0}$ & $14.2_{-0.0}^{+0.0}$\\[2pt]
$158.60_{-0.00}^{+0.00}$ & $-3.97_{-0.02}^{+0.02}$ & $0.21_{-0.01}^{+0.02}$ & $21.20_{-0.05}^{+0.05}$ & $3.24_{-0.03}^{+0.02}$ & $-0.50_{-0.05}^{+0.05}$ & $6.6_{-0.0}^{+0.1}$ & $5.3_{-0.2}^{+0.1}$ & $8.4_{-0.1}^{+0.1}$\\[2pt]
$192.58_{-0.01}^{+0.01}$ & $-3.93_{-0.05}^{+0.03}$ & $0.19_{-0.01}^{+0.02}$ & $21.19_{-0.06}^{+0.07}$ & $3.30_{-0.05}^{+0.04}$ & $-0.48_{-0.06}^{+0.07}$ & $4.3_{-0.0}^{+0.0}$ & $5.7_{-0.3}^{+0.3}$ & $7.1_{-0.2}^{+0.2}$\\[2pt]
$209.68_{-0.22}^{+0.15}$ & $0.70_{-0.22}^{+0.16}$ & $-2.40_{-0.07}^{+0.09}$ & $13.98_{-0.19}^{+0.23}$ & $3.46_{-0.34}^{+0.35}$ & $-2.83_{-0.33}^{+0.36}$ & $4.1_{-1.0}^{+0.6}$ & $6.9_{-2.2}^{+3.4}$ & $8.0_{-1.5}^{+2.8}$\\[2pt]

